Incentivizing Exploration with Heterogeneous Value of Money

Recently, Frazier et al. proposed a natural model for crowdsourced exploration of different a priori unknown options: a principal is interested in the long-term welfare of a population of agents who arrive one by one in a multi-armed bandit setting. However, each agent is myopic, so in order to incentivize him to explore options with better long-term prospects, the principal must offer the agent money. Frazier et al. showed that a simple class of policies called time-expanded are optimal in the worst case, and characterized their budget-reward tradeoff. The previous work assumed that all agents are equally and uniformly susceptible to financial incentives. In reality, agents may have different utility for money. We therefore extend the model of Frazier et al. to allow agents that have heterogeneous and non-linear utilities for money. The principal is informed of the agent's tradeoff via a signal that could be more or less informative. Our main result is to show that a convex program can be used to derive a signal-dependent time-expanded policy which achieves the best possible Lagrangian reward in the worst case. The worst-case guarantee is matched by so-called "Diamonds in the Rough" instances; the proof that the guarantees match is based on showing that two different convex programs have the same optimal solution for these specific instances. These results also extend to the budgeted case as in Frazier et al. We also show that the optimal policy is monotone with respect to information, i.e., the approximation ratio of the optimal policy improves as the signals become more informative.

==> app-DitR.tex <==
\section{Diamonds in the Rough: Proof of Theorem \ref{theorem:last_imposs}}
\label{app:last_imposs}

\begin{proof}
Lemma~\ref{lemma:imposs} showed that for every signaling scheme,
there is a $\theB$ (a parameter of the non-constant arms) such that
$\qStar$ and $\qHat$ coincide on the MAB instance \Dime. 
% \dkdelete{Note that this \emph{does not} mean that the policy
% $\textbf{TES}^\ast$ (parameterized by $\qStar$) runs exactly the same
% as the $\mathcal{A}(\qHat)$ (as it turns out later they have the same
% performance).}
It remains to show that these instances are in fact worst-case
instances, i.e., that the ratio between
$\DR_{\lambda}(\mathcal{A}(\qHat))$ and $\opt_\gamma$ in \Dime is
exactly $1 - p^\ast \gamma$.

First note that $\opt_\gamma = \frac{\theB}{1 - \gamma}$:
once a non-constant arm falls into a good state, it is optimal to
pull that arm forever.
We next show that 
$\DR_{\lambda}(\mathcal{A}(\qHat)) 
= \frac{\theB \cdot (1 - p^\ast \gamma)}{1 - \gamma}$.
  %It is not clear how to directly analyze the performance of $\textbf{TES}^\ast$ on Diamonds-in-the-rough instance, but, $\mathcal{A}(\qHat)$ is the optimal policy \emph{with payments} and therefore $\DR_{\lambda}(\textbf{TES}^\ast) \le \DR_{\lambda}(\mathcal{A}(\qHat))$.
Thereto, we use both convex programs and the fact that 
$\qHat = \qStar$. 
Substituting $\qStar$ into the objective of
program~\eqref{program:dp}, we obtain the following Lagrangian reward
for the time-expanded policy:

\begin{align*}
\DR_{\lambda}(\mathcal{A}(\qHat)) 
& = \frac{1}{1 - \gamma} \Big((1 - \gamma) \sumSig \SP{s} q^\ast_s + \sumSig \SP{s} ( 1- q^\ast_s)(\theB -\lambda \frac{(1-\gamma)(1 - \theB)}{\inv{F_s}(q^\ast_s)})\Big).
\end{align*}

The non-trivial constraint of program \eqref{program:main} has to be
tight; otherwise, the objective could be increased by lowering
individual $q^*_s$ values.
Therefore, $\sum_{s \in \sigSpace} \SP{s} q^\ast_s 
= \lambda \sum_{s \in \sigSpace} \SP{s} \frac{1 - q^\ast_s}{F_s^{-1}(q^\ast_s)}$,
which allows us to simplify the previous expression to
\begin{align*}
\DR_{\lambda}(\mathcal{A}(\qHat))
& = \frac{\theB (1 - p^\ast \gamma)}{1 - \gamma}
\; = \;  (1 - p^\ast \gamma) \cdot \opt_\gamma.
\end{align*} 
Therefore, on this instance,
$\DR_{\lambda}(\textbf{TES}^\ast) \leq (1 - p^\ast \gamma) \opt_\gamma$. 
By Theorem \ref{theorem:main_algo},  this bound is tight.
 \end{proof}
% \dkdelete{we also know that $\DR_{\lambda}(\textbf{TES}^\ast) \ge (1 - p^\ast \gamma) \opt_\gamma$, so it is actually an equality. As a by-product, this also shows that the approximation ratio of $\textbf{TES}^\ast$ is tight.}


==> app-concave-linear.tex <==
\section{Reducing Concave Money Value to Linear Money Value}
\label{app:concave-linear}
\newcommand{\Done}[1][]{\ensuremath{\ifthenelse{\equal{#1}{}}{\mathcal{D}^1}{\mathcal{D}^1_{#1}}}\xspace}
\newcommand{\Dtwo}[1][]{\ensuremath{\ifthenelse{\equal{#1}{}}{\mathcal{D}^2}{\mathcal{D}^2_{#1}}}\xspace}
\def\scaleC{\ensuremath{C}\xspace}
\def\mDiff{\xi}

In this section, we show that among concave \MUFs, linear functions
obtain the worst-case approximation ratio. 
This shows that our assumption that agents have linear \MUFs is
without loss of generality. 
We fix the distribution (or prior) over agents and the signaling
scheme and then perform a worst-case analysis over MAB instances.
The intuition is that the rewards of an MAB instance can be scaled up
so large that only the asymptotic behavior of concave \MUFs matters.

For any \MUF $\MF$, define 
$r_{\MF} = \lim_{x \to \infty} \frac{\MF(x)}{x}$
to be the limiting slope\footnote{%
As $\MF$ is concave, this limit always exists and is finite.}
of $\MF$, 
and $d_{\MF} = \inf \Set{t \ge 0}{r_{\MF} x + t \geq \MF(x) \text{ for
    all } x \geq 0}$ the minimum intercept.
Thus, we ensure that for all $x$:
\[ 
r_{\MF} x \; \leq \; \Mf{x} \; \leq \; d_{\MF} + r_{\MF} x.
\]

Fix a signaling scheme $\sigSch$.
For a given signal $s$ and its original posterior distribution $F_s$
over concave functions, define two distributions over affine functions.
Under \Done[s], each function $\MF$ is mapped to the linear function
$x \mapsto r_{\MF} \cdot x$.
Under \Dtwo[s], the function $\MF$ is mapped to the function
$x \mapsto d_{\MF} + r_{\MF} \cdot x$.
We assume that \Done[s] is a continuous distribution for each $s$.

Our proof breaks into two parts: lower bound (algorithm) and upper
bound (impossibility). 

\textbf{Lower bound}: 
Given the true distribution $(F_s)_{s \in \sigSpace}$ over concave
functions, instead compute the optimal policy for 
$(\Done[s])_{s \in \sigSpace}$. 
Because $r_{\MF} \cdot x \leq \Mf{x}$ for all $x$, each agent likes money
more under $\MF$ than under $r_{\MF}$. 
Thus, coupling the choices of agents between the two distributions,
each agent who plays non-myopically under the policy for $\Done$ also
does so under $F$, and at the same price.
Because the probability of playing myopically can only decrease, the
approximation guarantee $(1 - p^\ast(\sigSch) \gamma)$ can only increase.

\textbf{Upper bound}:
Next we show that in the worst case, the distribution $(F_s)$ over
concave functions does not yield a better approximation guarantee than
$(\Done[s])$.
First, notice that by the same argument as the previous paragraph, the
principal's utility under $(F_s)$ is upper bounded by his utility with
a distribution $(\Dtwo[s])_{s \in \sigSpace}$ over affine functions.
We will upper-bound the worst-case utility under $(\Dtwo[s])$ in terms
of that under $(\Done[s])$.

Thereto, we modify the Diamonds-in-the-rough instance from
Section~\ref{sec:diamond}, by scaling all reward values by some large
constant $\scaleC$. 
Let $\mDiff = C(1 - \gamma)(1 - \theB)$ be the difference between the
reward of the myopic arm and the Gittins arm. 
We will prove that for some carefully chosen constant $\scaleC$, the
optimal policy with payments for $\Dtwo$ cannot achieve much more than
the optimum for $\Done$. 
Let $(c_s)_s$ be the payments offered under different signals under
the optimal solution $\Dtwo$.

By the argument preceding the program \eqref{program:dp},
the optimum solution for $\Dtwo$ maximizes
\begin{equation}
C (1 - \gamma) \cdot 
\sum_s \SP{s} \cdot \Prob[(r,d) \sim {\Dtwo[s]}]{r \cdot c_s + d \leq \mDiff}
+ \sum_s \SP{s} \cdot (1 - \Prob[(r,d) \sim {\Dtwo[s]}]{r \cdot c_s + d \leq \mDiff})(C \cdot B - \lambda c_s),
\label{eqn:dtwo-optimization}
\end{equation}
while the optimum solution for $\Done$ maximizes
\begin{equation}
C (1 - \gamma) \cdot 
\sum_s \SP{s} \cdot \Prob[r \sim {\Done[s]}]{r \cdot c_s \leq \mDiff}
+ \sum_s \SP{s} \cdot (1 - \Prob[r \sim {\Done[s]}]{r \cdot c_s \leq \mDiff})(C \cdot B - \lambda c_s).
\label{eqn:done-optimization}
\end{equation}

Now, for any arbitrarily small $\epsilon$, focus on a finite set
$\sigSpace'$ of signals which together contribute at least a $(1-\epsilon)$
fraction of the optimum utility under both $\Done$ and $\Dtwo$. 
Note that such a set must always exist, because we assumed that the
signal space is countable; by sorting the signals by their
contribution and taking prefixes in this ordering, we see that the
total utility of these prefixes must converge to the overall total
utility as the size of the prefix grows. 

For each individual signal $s$, the optimal $c_s \to \infty$
as $\scaleC \to \infty$. 
Thus, because $\sigSpace'$ is finite,
for any desired lower bound $\alpha$, there exists a $\scaleC$ 
such that $c_s \geq \alpha$ for all $s \in \sigSpace'$.
Similarly, for any $\epsilon > 0$, there is a (sufficiently large)
$\beta$ such that
$\Prob[(r,d) \sim {\Dtwo[s]}]{d \leq \beta} \geq 1 - \epsilon$ 
holds simultaneously for all $s \in \sigSpace'$.
Given a target $\epsilon$, we first choose a suitable $\beta$, and
then choose $\scaleC$ to ensure that $\alpha \gg \beta$.
Then, we get that for all $s \in \sigSpace'$,

\begin{align*}
\Prob[(r,d) \sim {\Dtwo[s]}]{r c_s + d \leq \mDiff} 
& = \Prob[(r,d) \sim {\Dtwo[s]}]{r \leq \frac{\mDiff - d}{c_s}}\\
& \geq (1-\epsilon) \cdot 
\Prob[(r,d) \sim {\Dtwo[s]}]{r \leq \frac{\mDiff}{c_s} - \frac{\beta}{\alpha}}\\
& = (1-\epsilon) \cdot 
\Prob[r \sim {\Done[s]}]{r \leq \frac{\mDiff}{c_s} - \frac{\beta}{\alpha}}.
\end{align*}

Because we assumed that $\Done[s]$ is continuous for each $s$, 
we obtain that for each $s$,
by choosing $\alpha \gg \beta$ large enough (ensured by making
$\scaleC$ large enough), we get that
$\Prob[r \sim {\Done[s]}]{r \leq \frac{\mDiff}{c_s} - \frac{\beta}{\alpha}}
\geq \Prob[r \sim {\Done[s]}]{r \leq \frac{\mDiff}{c_s}} - \epsilon$.
By choosing $\scaleC$ as the maximum of the corresponding values, this
inequality holds simultaneously for all $s$.
In summary, we obtain that
%As semi-regularity implies continuity, we can increase $\scaleC$ even further to ensure that $\Prob[(r,d) \sim {\Dtwo[s]}]{r c_s + d \leq \mDiff} \ge (1-\epsilon) \cdot (\Prob[(r,d) \sim {\Dtwo[s]}]{r \leq \frac{\mDiff}{c_s}} - \epsilon)$ for all $s \in \sigSpace'$. This implies that 
\[
\Prob[(r,d) \sim {\Dtwo[s]}]{r c_s + d \leq \mDiff}
\geq 
\Prob[r \sim {\Dtwo[s]}]{r c_s \leq \mDiff} + 2\epsilon.
\]

Substituting this inequality into the objective value
\eqref{eqn:dtwo-optimization} show that the objective values 
\eqref{eqn:dtwo-optimization} and \eqref{eqn:done-optimization}
differ by at most
%Such difference in the value of probability will cause a change in the objective of $\opt(\Dtwo)$ of value at most:
\[
  \sum_s \SP{s} \cdot (|C(1 - \gamma - B)| \cdot 2\epsilon + \lambda \beta)
\; = \; |C(1 - \gamma - B)| \cdot 2\epsilon + \lambda \beta.
\]

% Recall that $c_s$ the optimal for $\opt(\Dtwo)$ and that $\Prob[(r,d) \sim {\Dtwo[s]}]{r \leq \frac{\mDiff}{c_s}} = \Prob[r \sim {\Done[s]}]{r \cdot c_s \leq \mDiff}$,

%\begin{equation}
%\opt(\Dtwo) = C (1 - \gamma) \cdot 
%\sum_s \SP{s} \cdot \Prob[(r,d) \sim {\Dtwo[s]}]{r \cdot c_s + d \leq \mDiff}
%+ \sum_s \SP{s} \cdot (1 - \Prob[(r,d) \sim {\Dtwo[s]}]{r \cdot c_s + d \leq \mDiff})(C \cdot B - \lambda c_s)
%\end{equation}
%\begin{equation}
%\le C (1 - \gamma) \cdot 
%\sum_s \SP{s} \cdot \Prob[r \sim {\Done[s]}]{r \cdot c_s \leq \mDiff}
%+ \sum_s \SP{s} \cdot (1 - \Prob[r \sim {\Done[s]}]{r \cdot c_s \leq \mDiff})(C \cdot B - \lambda c_s) + C(1 - \gamma - B) 2\epsilon + \lambda \beta.
%\end{equation}

The optimum value of the objective \eqref{eqn:done-optimization}
grows at least linearly in $C$. 
The reason is that when $C$ is scaled up by any constant $\nu$, a
feasible solution is obtained by scaling all $c_s$ up by $\nu$ as
well; this results in a multiplicative increase of $\nu$ in the
objective value. Thus, the \emph{best} $c_s$ values must attain at
least such an increase.
Because the error term $C(1 - \gamma - B) 2\epsilon + \lambda \beta$
is at most $O(\epsilon) \cdot \opt(\Done)$, we obtain that
\[
\opt(\Dtwo) \; \leq \; \opt(\Done) \cdot (1 + O(\epsilon)).
\]
Finally, adding in the $O(\epsilon)$ terms for signals not considered
in this argument does not change the above conclusion.
Making $\epsilon$ arbitrarily small (and scaling the
Diamonds-in-the-Rough instance correspondingly) then shows in the
limit that the distributions over linear and affine functions have the
same worst-case behavior.

==> app-garbling.tex <==
\section{Signal Garbling: Proof of Theorem~\ref{theorem:garbling_at_intro}}
\label{sec:app_garbling}
% In this section, we show that if we garble a signalling scheme
% $\sigSch$ into $\sigSch'$, the optimal approximation ratio for garbled signaling scheme $\sigSch'$ is worse. Here by
% garbling we mean (stochastically) mapping each signal in $\sigSch$ to a random (new) signal in $\sigSch'$. \citet{marschak1968economic} gave a
% formal definition (rephrased to fit our model) as follows:

% \begin{definition}
%   A signaling scheme $\sigSch'$ is a garbled verion of signaling scheme $\sigSch$ if for all \Umr $r$, signal $s\in \sigSpace$ , $s'\in \sigSpace'$ the following conditions hold,
%   \begin{itemize}
%   \item $\ProbC{s'}{s, r} = \ProbC{s'}{s}$;
%   \item $f(r|s,s')  = f(r|s)$, $f(r|\cdot)$ is the conditional pdf of \Umr $r$;
%   \item $\ProbC{s,s'}{r} = \ProbC{s}{r} \cdot \ProbC{s'}{s}$.
%   \end{itemize}
% where  $\sigSpace,
% \sigSpace'$ are the signaling spaces of $\sigSch$ and $\sigSch'$
% respectively.
% \end{definition}

In this section, we provide the proof of 
Theorem~\ref{theorem:garbling_at_intro}.
We restate it here for convenience.

\begin{rtheorem}{Theorem}{\ref{theorem:garbling_at_intro}}
Let $\sigSch$ and $\sigSch'$ be two signaling schemes such that
$\sigSch'$ is a garbling of $\sigSch$.
Then, $1 - p^\ast(\sigSch) \gamma \geq 1 - p^\ast(\sigSch') \gamma$. 
\end{rtheorem}

\begin{proof}
Let $\SP{s}, \SP{s'}$ be the unconditional probabilities of observing
signals $s,s'$, as defined as in Section~\ref{sec:prelim-signaling},
and let $(\MP{s'})_{s'\in \sigSpace'}$ be the optimal solution for
program \eqref{program:main} with signaling scheme $\sigSch'$.
We will show that the program \eqref{program:main} for signaling
scheme $\sigSch$ has a feasible solution $(\MP{s})_{s\in \sigSpace}$ 
such that 
$\sum_{s\in \sigSpace} \SP{s}\MP{s} =
\sum_{s'\in \sigSpace'} \SP{s'}\MP{s'}$.
This implies that the policy with the garbled signaling scheme cannot
outperform the policy with the original signaling scheme.

Let $\SP{s,s'}$ be the (joint) probability that signal $s$ is revealed
by $\sigSch$ and signal $s'$ is revealed by the garbling $\sigSch'$. 
Thus, $\SP{s'} = \sum_{s\in\sigSpace}\SP{s,s'}$.
Conditioned on the two revealed signals $s,s'$, let 
$\MP{s,s'}$ be the probability that the policy with parameters
$(\MP{s'})_{s' \in \sigSpace}$ (which only observes $s'$) 
obtains a myopic arm pull. Notice that this probability depends
on $s$: while $s$ does not affect the threshold that is set by the
policy, it does affect the distribution of the agent's \Umr, and hence
the probability of a myopic pull.
Thus, the overall probability of a myopic pull with signal $s'$ can be
obtained by summing over all (unobserved) signals $s$ as
$\SP{s'} \MP{s'} = \sum_{s\in \sigSpace}\SP{s,s'} \MP{s,s'}$.

Since $\MP{s'}$ is a feasible solution of \eqref{program:main}, we have 
\[
  \sum_{s'\in \sigSpace'} \SP{s'} \MP{s'} 
\geq \lambda\sum_{s'\in \sigSpace'} \SP{s'} \frac{1-\MP{s'}} {F_{s'}^{-1}(\MP{s'})}.
\]

Substituting $\SP{s'} = \sum_{s\in\sigSpace}\SP{s,s'}$
and $\MP{s'} = \frac{\sum_{s\in \sigSpace}\SP{s,s'} \MP{s,s'}}{\SP{s'}}$,
we can write

\[
\SP{s'} \cdot \frac{1-\MP{s'}}{F_{s'}^{-1}(\MP{s'})}
\; = \; \frac{\SP{s'}}{F_{s'}^{-1}(\MP{s'})} \cdot
  (1-\frac{\sum_{s\in \sigSpace}\SP{s,s'}\MP{s,s'}}{\SP{s'}})\\
\; = \; \sum_{s\in \sigSpace}
   \SP{s,s'} \cdot \frac{1-\MP{s,s'}}{F_{s'}^{-1}(\MP{s'})}.
\]


Next, we observe that $F_{s}^{-1}(\MP{s,s'}) = F_{s'}^{-1}(\MP{s'})$,
as follows:
because $\sigSch'$ is a garbling of $\sigSch$, we get that
the conditional distributions satisfy $F_s(r) = F_{s,s'}(r)$.
$F_{s'}^{-1}(\MP{s'}) =: \tau$ is a threshold chosen by the mechanism
with knowledge solely of $s'$, chosen to achieve a probability of
myopic play of exactly $\MP{s'}$.
$\MP{s,s'}$ denotes the probability of myopic play with this threshold
$\tau$, with the additional knowledge that the ungarbled signal was
$s$. 
Thus, we obtain that $\MP{s,s'} = F_{s,s'}(\tau) = F_s(\tau)$,
by the garbling property. 
Taking inverses now shows that
$F_{s'}^{-1}(\MP{s'}) = \tau = F_{s}^{-1}(\MP{s,s'})$.

Now define the target probabilities for the ungarbled signals as follows:
$\MP{s} =\sum_{s' \in \sigSpace'} \frac{\SP{s,s'}}{\SP{s}} \cdot \MP{s,s'}$.
We can then write

\begin{align*}
\sum_{s\in \sigSpace} \SP{s}\MP{s} 
& = \sum_{s \in \sigSpace} \sum_{s' \in \sigSpace'} \SP{s,s'}\MP{s,s'} \\
& = \sum_{s' \in \sigSpace'} \sum_{s \in \sigSpace} \SP{s,s'}\MP{s,s'} \\
& \geq \lambda \sum_{s' \in \sigSpace'} \sum_{s \in \sigSpace}
  \SP{s,s'} \cdot \frac{1-\MP{s,s'}}{F_{s}^{-1}(\MP{s,s'})}\\
& = \lambda \sum_{s \in \sigSpace} \sum_{s' \in \sigSpace'}
  \SP{s} \cdot \frac{\SP{s,s'}}{\SP{s}} \cdot
  \frac{1-\MP{s,s'}}{F_{s}^{-1}(\MP{s,s'})}\\
& \stackrel{(*)}{\geq} \lambda \sum_{s \in \sigSpace} \SP{s} \cdot 
  \frac{1-\sum_{s' \in \sigSpace'} \frac{\SP{s,s'}}{\SP{s}} \MP{s,s'}}{%
  F_{s}^{-1}(\sum_{s' \in \sigSpace'} \frac{\SP{s,s'}}{\SP{s}} \cdot \MP{s,s'})}\\
& = \lambda \sum_{s \in \sigSpace} 
  \SP{s} \cdot \frac{1-\MP{s}}{F_{s}^{-1}(\MP{s})}.
\end{align*}
Here, the inequality labeled (*) followed by semi-regularity of $F_s$.
The inequality derived above implies that $\MP{s}$ is a feasible
solution of \eqref{program:main} with signaling scheme $\sigSch$, and
it attains at least the same utility for the principal.
This completes the proof of the theorem.
\end{proof}

%\begin{align*}
%  \sum_{s'\in \sigSpace'} \sum_{s\in \sigSpace} \SP{s,s'}\MP{s,s'}
%&\ge \lambda\sum_{s'\in \sigSpace'} \SP{s'}\frac{1-\MP{s'}}{F_{s'}^{-1}(\MP{s'})} \\
%&= \lambda\sum_{s'\in \sigSpace'}
%  \frac{\SP{s'}}{F_{s'}^{-1}(\MP{s'})}(1-\frac{\sum_{s\in
%  \sigSpace}\SP{s,s'}\MP{s,s'}}{\SP{s'}})\\
%&=\lambda\sum_{s'\in \sigSpace'} \sum_{s\in
%  \sigSpace}\SP{s,s'}\frac{1-\MP{s,s'}}{F_{s'}^{-1}(\MP{s'})}\\
%&=\lambda\sum_{s'\in \sigSpace'} \sum_{s\in
%  \sigSpace}\SP{s,s'}\frac{1-\MP{s,s'}}{F_{s}^{-1}(\MP{s,s'})}
%\end{align*}


%\begin{align*}
%\sum_{s\in \sigSpace} \sum_{s'\in \sigSpace'} \SP{s,s'}\MP{s,s'} 
%&\ge \lambda \sum_{s\in \sigSpace} \sum_{s'\in
%  \sigSpace'}\SP{s,s'}\frac{1-\MP{s,s'}}{F_{s}^{-1}(\MP{s,s'})}\\
%&= \lambda\sum_{s\in \sigSpace} \sum_{s'\in
%  \sigSpace'}\SP{s}\ProbC{s'}{s}\frac{1-\MP{s,s'}}{F_{s}^{-1}(\MP{s,s'})}\\
%&\ge \lambda \sum_{s\in \sigSpace} \SP{s}\frac{1-\sum_{s'\in
%  \sigSpace'}\ProbC{s'}{s}\MP{s,s'}}{F_{s}^{-1}(\sum_{s'\in
%  \sigSpace'}\ProbC{s'}{s}\MP{s,s'})}
%\end{align*}



==> app-lb.tex <==

% \section{Time Expansion: Missing Proofs from Section \ref{sec:algo}}
% \label{app:algo}
The proofs are very straightforward (syntactic) modifications of those of the corresponding lemmas in \cite{original}, we include them here for completeness. 

% \begin{rtheorem}{Lemma}{\ref{lem:TE}} 
% Fix a signaling scheme $\sigSch$. If $\MPV$ satisfies $\sum_{s \in
%     \sigSpace} \SP{s} \MP{s} \ge\lambda\sum_{s \in \sigSpace} \SP{s} \frac{1 -
% \MP{s}}{F_s^{-1} (\MP{s})}$,  there exists a policy $\ALG$, 
% such that the time-expanded policy $\Te{q}{A}$ satisfies
% \begin{equation}
% \DR_{\lambda}(\Te{q}{A}) 
% \geq (1 - \gamma \cdot \sum_{s \in \sigSpace} \SP{s} \MP{s}) \cdot \opt_{\gamma}.
% \end{equation}
% %where $p=\sum_{s\in \sigSpace} \SP{s} \MP{s}$ is the unconditional probability that the
% %myopic arm is pulled by the agent.
% \end{rtheorem}

\begin{rtheorem}[Modification of Lemma 4.2 of \cite{original}]{Lemma}{\ref{cite42}}
Given a parameter $\lambda$ and a signaling scheme $\sigSch$. Let $\zeta_{t-1}=\sum_{t'<t}Z_{t'}$ be the total
number of non-myopic steps performed by the time-expanded algorithm $\Te{\MPV}{A}$
prior to time $t$, where $\MPV$  satisfies
$\sum_{s \in \sigSpace} \SP{s} \MP{s} \ge\lambda\sum_{s \in \sigSpace}
\SP{s} \frac{1 -\MP{s}}{F_s^{-1} (\MP{s})}$. 
Then, for any $0\le n\le t$,
\begin{align*}
\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t}-\lambda\payment{t}{i_t}}{\zeta_{t-1} = n}
& \ge \Expect[\ALG]{\reward{n}{i_n}}.
\end{align*}
\end{rtheorem}

\begin{proof}
The Lagrangian utility at time $t$ is 
$\reward{t}{i_t} - \lambda\payment{t}{i_t}$.
Let $x = \max_i \ExpectC{\reward{t}{i}}{\ve{S}_t,\Zed_{0:t-1}}$ 
and $y = \ExpectC{\reward{t}{i_t^\ast}}{\ve{S}_t,\Zed_{0:t-1}}$, 
where $\Zed_{0:t-1}=(\Zed_0,\Zed_t,\dots,\Zed_{t-1})$. 
Since the myopic arm is played with probability $\MP{s}$,
the expected Lagrangian utility will be 
\begin{align*}
\ExpectC[{\Te{q}{A}}]{\reward{t}{i_t} - \lambda \payment{t}{i_t}}{\ve{S}_t, \Zed_{0:t-1}}&= \sum_{s\in\sigSpace}\SP{s}(\MP{s} x +
(1-\MP{s})(y-\lambda\frac{x-y}{F_s^{-1}(\MP{s})}) )\\
% &=x\sum_{s\in \sigSpace} \SP{s}(\MP{s}-   \frac{\lambda(1 -
% \MP{s})}{F_s^{-1} (\MP{s})})  \\ &
% + y\sum_{s\in \sigSpace}
% \SP{s}(1-\MP{s}+\frac{\lambda(1-\MP{s})}{F_s^{-1} (\MP{s})})\\
&= y\sum_{s\in \sigSpace} \SP{s} + (x-y)\sum_{s\in\sigSpace}\SP{s}(\MP{s} -
\frac{\lambda(1-\MP{s})}{F_s^{-1} (\MP{s})}) \ge y.
\end{align*}

The last inequality above is due to $x\ge y$ 
(by the myopic arm preference) and 
$\sum_{s \in \sigSpace} \SP{s} \MP{s} \ge\lambda\sum_{s \in \sigSpace}
\SP{s} \frac{1 - \MP{s}}{F_s^{-1} (\MP{s})}$ (by assumption of the lemma).
Notice how the condition 
$\sum_{s \in \sigSpace} \SP{s} \MP{s} \ge\lambda\sum_{s \in \sigSpace} \SP{s} \frac{1 - \MP{s}}{F_s^{-1} (\MP{s})}$ in the
statement of the lemma allowed us the cancel out the myopic
arm-rewards $x$, which would otherwise have been difficult to analyze.
Now we have $$\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t}- \lambda \payment{t}{i_t}}{\ve{S}_t, \Zed_{0:t-1}} \geq
\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t^\ast}}{\ve{S}_t, \Zed_{0:t-1}}.$$

Since the expected reward only depends on the current state of arm
$\ve{S}_t$, we can add the status of previous round to the condition, 
$$\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t}- \lambda \payment{t}{i_t}}{\ve{S}_{0:t}, \Zed_{0:t-1}} \geq
\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t^\ast}}{\ve{S}_{0:t},
  \Zed_{0:t-1}}.$$

Taking conditional expectation on both sides with the condition
$\hat{\ve{S}}_t, \zeta_{t-1} = n$,

\begin{align*}
 \ExpectC[\Te{\MPV}{A}]{\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t}- \lambda
   \payment{t}{i_t}}{\ve{S}_{0:t}, \Zed_{0:t-1}}}{\hat{\ve{S}}_t,\zeta_{t-1} = n} \\
\geq
\ExpectC[\Te{\MPV}{A}]{\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t^\ast}}{\ve{S}_{0:t}, \Zed_{0:t-1}}}{\hat{\ve{S}}_t, \zeta_{t-1} = n}.
\end{align*}

Since $\hat{\ve{S}}_t, \zeta_{t-1} = n$ is measurable by
$\ve{S}_{0:t}, \Zed_{0:t-1}$, we can use the tower property of
conditional expectations and get
$$\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t}- \lambda
  \payment{t}{i_t}}{\hat{\ve{S}}_t,\zeta_{t-1} = n} \geq
\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t^\ast}}{\hat{\ve{S}}_t, \zeta_{t-1}
  = n}.$$

Let $\tau\ge t$ be the next time when $\Te{\MPV}{A}$ performs a
non-myopic pull. Since the reward sequence for each arm forms a
Martingale, and $i_u^\ast$ is fixed with a certain $\hat{\ve{S}}_t$,
we have that $\ExpectC[\Te{\MPV}{A}]{\reward{u}{i_{u}^\ast}}{\hat{\ve{S}}_t,
\zeta_{t-1} = n}$ is identical for all $u\ge t$. Now if we write $\ExpectC[\Te{\MPV}{A}]{\reward{\tau}{i_{\tau}^\ast}}{\hat{\ve{S}}_t,
\zeta_{t-1} = n}$ with the law of total probability, we have

\begin{align*}
 \ExpectC[\Te{\MPV}{A}]{\reward{\tau}{i_{\tau}^\ast}}{\hat{\ve{S}}_t,\zeta_{t-1}
  = n} &= \sum_{u\ge t}\Prob{\tau = u}\cdot
  \ExpectC[\Te{\MPV}{A}]{\reward{u}{i_{u}^\ast}}{\hat{\ve{S}}_t,\zeta_{t-1}
  = n, \tau = u} \\
&  = \ExpectC[\Te{\MPV}{A}]{\reward{t}{i_{t}^\ast}}{\hat{\ve{S}}_t,\zeta_{t-1}
  = n} .
\end{align*}

So far, we have proved that $$\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t}- \lambda
  \payment{t}{i_t}}{\hat{\ve{S}}_t,\zeta_{t-1} = n} \geq
\ExpectC[\Te{\MPV}{A}]{\reward{\tau}{i_\tau^\ast}}{\hat{\ve{S}}_t, \zeta_{t-1}
  = n}.$$

Taking conditional expectations with respect to $\zeta_{t-1} = n$, then
applying the law of iterated expectation, 
$$\ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t}- \lambda
  \payment{t}{i_t}}{\zeta_{t-1} = n} \geq
\ExpectC[\Te{\MPV}{A}]{\reward{\tau}{i_\tau^\ast}}{\zeta_{t-1}
  = n}.$$
Note the right-hand side is exactly $\Expect[\ALG]{\reward{n}{i_n}}$ by
definition of $\Te{\MPV}{A}$,
finishing the proof.
\end{proof}

\begin{rtheorem}[Variation of Lemma 3.2 of \cite{original}]{Lemma}{\ref{cite32}}
Given a parameter $\lambda$ and a signaling scheme $\sigSch$.  Assume  $\MPV$ satisfies
$\sum_{s \in \sigSpace} \SP{s} \MP{s} \ge\lambda\sum_{s \in \sigSpace}
\SP{s} \frac{1 -\MP{s}}{F_s^{-1} (\MP{s})}$, then for $\eta =
\frac{(1-p)\gamma}{1-p\gamma}$, where $p=\sum_{s\in \sigSpace}\SP{s}\MP{s}$, we have 
\begin{align*}
R_{\lambda}^{(\gamma)}(\Te{\MPV}{A})
& \ge \frac{1-\eta}{1-\gamma}\cdot R^{(\eta)}(\ALG).
\end{align*}
\end{rtheorem}

\begin{proof}
  \begin{align*}
    R_{\lambda}^{(\gamma)}(\Te{\MPV}{A})\quad &=\quad &&\sum_{t=0}^\infty \gamma^t
                                        \Expect[\Te{\MPV}{A}]{\reward{t}{i_t}-
                                        \lambda\payment{t}{i_t}}\\
    &= &&\sum_{t=0}^\infty\sum_{n=0}^\infty\gamma^t \ExpectC[\Te{\MPV}{A}]{\reward{t}{i_t}- \lambda
  \payment{t}{i_t}}{\zeta_{t-1} =n} \cdot \Prob{\zeta_{t-1} = n}\\
&\stackrel{\mathclap{\mbox{Lemma~\ref{cite42}}}}{\ge}&&\sum_{n=0}^\infty
  \Expect[\ALG]{\reward{n}{i_n}}\cdot\sum_{t=0}^\infty\gamma^t\cdot
  \Prob{\zeta_{t-1}=n}\\
&=&&\sum_{n=0}^\infty  \Expect[\ALG]{\reward{n}{i_n}}\cdot \sum_{t=0}^\infty\gamma^t\cdot
  \binom{t}{n}\cdot (1-p)^np^{t-n}\\
&=&&\sum_{n=0}^\infty  \Expect[\ALG]{\reward{n}{i_n}}\cdot \gamma^n
  (1-p)^n \cdot \sum_{i=0}^\infty
  \binom{n+i}{n}\cdot (\gamma p)^i\\
&=&&\sum_{n=0}^\infty  \Expect[\ALG]{\reward{n}{i_n}}\cdot \gamma^n
  (1-p)^n \cdot (1-\gamma p)^{-(n+1)}\\
&=&&\sum_{n=0}^\infty  \Expect[\ALG]{\reward{n}{i_n}}\cdot
  \frac{1-\eta}{1-\gamma}\cdot \eta^n.
  \end{align*}

In the penultimate step, we use $\sum_{i=0}^\infty \binom{n+i}{n} x^i
= (1-x)^{-(n+1)}$ for $n \ge 0$ and $|x|< 1$. 
\end{proof}


==> app-semi-regular.tex <==
\section{Semi-Regularity: Proof of Lemma~\ref{lemma:semireg}}
\label{sec:semi-reg-proof}
% Here, we provide proofs omitted from the main text.
% We begin by restating Lemma~\ref{lemma:semireg}.
\begin{rtheorem}{Lemma}{\ref{lemma:semireg}}
Let $G$ be the CDF of a non-negative random variable,
and define $\inv{G}(x) := sup \{ t \ge 0 : G(t) \le x \}$. 
If $\inv{G}(x) (1 - x)$ is concave, then
$\frac{1 - x}{\inv{G}(x)}$ is convex.
In particular, regularity implies semi-regularity.
\end{rtheorem}

\begin{proof}
  We only need to look at 3 points $x$, $\alpha x + (1 - \alpha)y$ and $y$, where $0 \le x < y \le 1$.
  Let $z = \alpha x + (1 - \alpha) y$
  By concavity of $\inv{G}(x) (1 - x)$, we have
  \begin{equation}
    \inv{G}(z) (1 - z) \ge \alpha \inv{G}(x)(1 - x) + (1 - \alpha)\inv{G}(y) (1 - y)
  \end{equation}
  Rearranging, we have:
  \begin{equation}
    0 \ge \alpha (1 - x) \frac{\inv{G}(x) - \inv{G}(z)}{\inv{G}(z)}
    + (1 - \alpha)(1 - y) \frac{\inv{G}(y) - \inv{G}(z)}{\inv{G}(z)}
  \end{equation}
  By monotonicity of $\inv{G}$, $\inv{G}(x) \le \inv{G}(z) \le \inv{G}(y)$.
  This implies
  \begin{equation}
    \label{app:semi}
    0 \ge \alpha (1 - x) \frac{\inv{G}(x) - \inv{G}(z)}{\inv{G}(x)}
    + (1 - \alpha)(1 - y) \frac{\inv{G}(y) - \inv{G}(z)}{\inv{G}(y)},
   \end{equation}
   as $\inv{G}(x) \le \inv{G}(z)$ and $\inv{G}(y) \ge \inv{G}(z)$.
   One can see that inequality \eqref{app:semi} is equivalent to the convexity of $\frac{1 - x}{\inv{G}(x)}$.
\end{proof}

% Here we show the optimal policy with payments has a nice characterization.
% In the most general case, the principal is solving an MDP problem,
% but has to hire agents to take action for her.
% Each round a new agent arrives, and prefers the myopic action $a_m(s)$ of current state $s$.
% Let $A(s)$ be the action set of state $s$.

% With extra payments $c_a$ for action $a$, the agent chooses the maximizer of $R(s, a) + c_a$, where $R(s, a)$ is the reward for taking action $a$ in state $s$.

% As the MDP is explicitly given, we can solve the problem by LP:
% \begin{equation}
% V(s) = \max_{a_i \in A(s)} \{ \sum_{s'} P_{a_i}(s, s') [R(s, a_i) + \gamma V(s')] - \lambda [R(s, a_m(s)) - R(s, a_i)]\}
% \end{equation}
% where $\lambda$ is the Lagrangian factor of the principal.

% But, we can merge the terms $R(s, a_i)$ and $\lambda [r(s, a(s)) - r(s, a_i)]$ together, and this will give us a new MDP with new reward function $R'(s, a_i) := R(s, a(s)) - \lambda [r(s, a(s)) - r(s, a_i)]$.
% \begin{equation}
% V'(s) = \max_{a_i \in A(s)} \{ \sum_{s'} P_{a_i}(s, s') [R'(s, a_i) + \gamma V'(s')]\}
% \end{equation}

% What we just showed is that the "Lagrangian version of MDP with myopic agents" can be reduced to a normal MDP problem without agents.
% Note the transformation does not change the transition probabilities, so I claim the "MDP problem with agents" can be solved using Gittins policy.

% %This is true for all MDPs and the original problem is just an MDP with exponentially many states, with actions being which arm to pull.

% Next, we restate and prove the lemmas from Section~\ref{sec:full-information}.

% \begin{rtheorem}{Lemma}{\ref{lem:one-round-threshold}}
% Consider a single arm pull, and a value $q \in [0,1]$. 
% Among all policies that have this arm pull be myopic with
% probability $q$, the one minimizing expected cost is a threshold
% policy.
% \end{rtheorem}
% \begin{rtheorem}{Lemma}{\ref{lem:threshold}}
% The \lagobj of any time-expanded policy
% $\mathcal{P}$ of $\ALG$ is (weakly) dominated by that of a threshold
% policy.
% \end{rtheorem}

